PolyStan: PolyChord nested sampling and Bayesian evidences for Stan models

Sampling from multi-modal distributions and estimating marginal likelihoods, also known as evidences and normalizing constants, are well-known challenges in statistical computation. They can be overcome by nested sampling, which evolves a set of live points through a sequence of distributions upwards in likelihood. We introduce PolyStan -- a nested sampling inference engine for Stan. PolyStan provides a Stan interface to the PolyChord nested sampling algorithm using bridgestan. PolyStan introduces a new user-base to nested sampling algorithms and provides a black-box method for sampling from challenging distributions and computing marginal likelihoods. We demonstrate the robustness of nested sampling on several degenerate and multi-modal problems, comparing it to bridge sampling and Hamiltonian Monte Carlo.

==> jssifarxiv.tex <==
% jss versus arxiv

\newif\ifarxiv
\arxivtrue

\makeatletter
\AtEndPreamble{%
    \ifarxiv%
        % style
        
        \@nojsstrue
        
        % fonts
        
        \usepackage[utf8]{inputenc}
        \usepackage{fourier}
        \usepackage[scale=0.8]{GoMono}
        \usepackage[scaled=1.04]{biolinum}
        \usepackage[T1]{fontenc}
        \usepackage{microtype}
        
        % codes
        
        \usepackage{listings}
        \usepackage{everysel}
    
        \input{lang}

        \newenvironment{colormath}{\everymath{\color{comment}}}{\everymath{\color{black}}}
        
        \let\CodeInput\@undefined
        \let\endCodeInput\@undefined
        \lstnewenvironment{CodeInput}[1][Stan]
        {\lstset{language=#1}\everymath{\color{blue}}}
        {\everymath{\color{black}}}

        \let\CodeOutput\@undefined
        \let\endCodeOutput\@undefined
        \lstnewenvironment{CodeOutput}[1][bash]
        {\lstset{language=#1}\everymath{\color{blue}}}
        {\everymath{\color{black}}}

        \renewcommand{\code}[1][bash]{\lstinline[language=#1, mathescape]}

        \providecommand{\eprint}[2][]{[\texttt{\href{https://arxiv.org/abs/#2}{#2}]}}
        \providecommand{\urlprefix}{}

    \else%
    
        \let\@CodeInput\CodeInput
        \let\@endCodeInput\endCodeInput
        \renewenvironment{CodeInput}[1][none]{\@CodeInput}{\@endCodeInput}

        \let\@CodeOutput\CodeOutput
        \let\@endCodeOutput\endCodeOutput
        \renewenvironment{CodeOutput}[1][none]{\@CodeOutput}{\@endCodeOutput}

        \let\@code\code
        \renewcommand{\code}[1][]{\@code}

        \usepackage{microtype}
        \DisableLigatures[-]{family=tt*}

        \usepackage{verbatim} 
    
    \fi%
}
\makeatother

==> lang.tex <==
\usepackage{amsmath}

\usepackage{etoolbox}
\makeatletter
\patchcmd{\lsthk@TextStyle}{\let\lst@DefEsc\@empty}{}{}{\errmessage{failed to patch}}
\makeatother

% colors

\definecolor{comment}{HTML}{0000FF}
\definecolor{number}{HTML}{FF00FF}
\definecolor{string}{HTML}{FF00FF}
\definecolor{keyword}{HTML}{A020F0}
\definecolor{type}{HTML}{FF00FF}
\definecolor{import}{HTML}{008A8C}
\definecolor{prompt}{HTML}{BEBEBE}


\lstdefinelanguage{json}{
    postbreak=\mbox{$\hookrightarrow$},
    string=[s]{"}{"},
    comment=[l]{:\ "},
    morecomment=[l]{:\ +},
    morecomment=[l]{:\ -},
    morecomment=[l]{:\ 0},
    morecomment=[l]{:\ 1},
    morecomment=[l]{:\ 2},
    morecomment=[l]{:\ 3},
    morecomment=[l]{:\ 4},
    morecomment=[l]{:\ 5},
    morecomment=[l]{:\ 6},
    morecomment=[l]{:\ 7},
    morecomment=[l]{:\ 8},
    morecomment=[l]{:\ 9},
    morecomment=[s]{[}{]},
}

\lstdefinelanguage{none}{
}

\lstdefinelanguage{pso}{
    morecomment=[s]{_|}{_|},
    frame=none,
}

\lstdefinelanguage{bash} {
    keywords=[2]{data, random, polychord, output, random, polychord, output, sudo, mpirun, uname},
    alsoletter={.},
    keywords=[4]{.data.},
    comment=[l]{\#},
    numberstyle=\prompt,
    numbers=left,
    numbersep=5pt,
    xleftmargin=14.5pt,
    framexleftmargin=12pt,
}

\newcommand\prompt[1]{\color{prompt}{\$}}
\newcommand\pyprompt[1]{\color{prompt}{>\!>\!>}}
\newcommand\pycontin[1]{\color{prompt}{.\!.\!.}}


\lstdefinelanguage{Python3}[]{Python}{
    morekeywords={with, as},
    keywords=[2]{True, False},
    alsoletter={.},
    keywords=[3]{arviz, anesthetic, matplotlib.pyplot, anesthetic.utils},
    literate=%
    {0}{{{\color{number}{0}}}}1
    {1}{{{\color{number}{1}}}}1
    {2}{{{\color{number}{2}}}}1
    {3}{{{\color{number}{3}}}}1
    {4}{{{\color{number}{4}}}}1
    {5}{{{\color{number}{5}}}}1
    {6}{{{\color{number}{6}}}}1
    {7}{{{\color{number}{7}}}}1
    {8}{{{\color{number}{8}}}}1
    {9}{{{\color{number}{9}}}}1
    {0.}{{{\color{number}{0.}}}}2
    {1.}{{{\color{number}{1.}}}}2
    {2.}{{{\color{number}{2.}}}}2
    {3.}{{{\color{number}{3.}}}}2
    {4.}{{{\color{number}{4.}}}}2
    {5.}{{{\color{number}{5.}}}}2
    {6.}{{{\color{number}{6.}}}}2
    {7.}{{{\color{number}{7.}}}}2
    {8.}{{{\color{number}{8.}}}}2
    {9.}{{{\color{number}{9.}}}}2
    {plot_1d}{{{\color{black}{plot\_1d}}}}7
    {float64}{{{\color{black}{float64}}}}7,
}

\lstdefinelanguage{Python3Prompt}[]{Python3}{
    numberstyle=\pyprompt,
    numbers=left,
    numbersep=5pt,
    xleftmargin=24.5pt,
    framexleftmargin=22pt,
}

\lstdefinelanguage{cpp}{
    keywords=[2]{true, false}
}
\lstdefinelanguage{Stan}{
    keywords={functions, data, parameters, transformed, model, generated, quantities},
    keywords=[2]{int, real, array, lower, upper, vector, matrix, return},
    alsoletter={.},
    keywords=[3]{polystan.stanfunctions},
    otherkeywords={\#include, ~},
    morekeywords=[2]{\#include, ~},  
    comment=[l]{//},
    literate=%
    {0}{{{\color{number}{0}}}}1
    {1}{{{\color{number}{1}}}}1
    {2}{{{\color{number}{2}}}}1
    {3}{{{\color{number}{3}}}}1
    {4}{{{\color{number}{4}}}}1
    {5}{{{\color{number}{5}}}}1
    {6}{{{\color{number}{6}}}}1
    {7}{{{\color{number}{7}}}}1
    {8}{{{\color{number}{8}}}}1
    {9}{{{\color{number}{9}}}}1
    {0.}{{{\color{number}{0.}}}}2
    {1.}{{{\color{number}{1.}}}}2
    {2.}{{{\color{number}{2.}}}}2
    {3.}{{{\color{number}{3.}}}}2
    {4.}{{{\color{number}{4.}}}}2
    {5.}{{{\color{number}{5.}}}}2
    {6.}{{{\color{number}{6.}}}}2
    {7.}{{{\color{number}{7.}}}}2
    {8.}{{{\color{number}{8.}}}}2
    {9.}{{{\color{number}{9.}}}}2,
}

\lstset{
    basicstyle=\ttfamily\normalshape,
    commentstyle=\color{comment},
    keywordstyle=\color{keyword}\bfseries,
    keywordstyle=[2]\color{type},
    keywordstyle=[3]\color{import},
    keywordstyle=[4]\color{black},
    stringstyle=\color{string},
    numberstyle=\ttfamily\footnotesize\color{prompt},
    backgroundcolor=\color{white},
    rulecolor=\color{prompt},
    breakatwhitespace=false,
    breaklines=true,
    captionpos=t,
    numbers=none,
    keepspaces=true,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2,
    escapechar={@}, 
    lineskip={0pt},
    framerule=0.75pt,
    frame=single,
    xleftmargin=0.2cm,
    framesep=3pt,
    framexleftmargin=3pt,
    numbersep=10pt,
}




